3D-ZeF: A 3D Zebrafish Tracking Benchmark Dataset

In this work we present a novel publicly available stereo based 3D RGB dataset for multi-object zebrafish tracking, called 3D-ZeF. Zebrafish is an increasingly popular model organism used for studying neurological disorders, drug addiction, and more. Behavioral analysis is often a critical part of such research. However, visual similarity, occlusion, and erratic movement of the zebrafish makes robust 3D tracking a challenging and unsolved problem. The proposed dataset consists of eight sequences with a duration between 15-120 seconds and 1-10 free moving zebrafish. The videos have been annotated with a total of 86,400 points and bounding boxes. Furthermore, we present a complexity score and a novel open-source modular baseline system for 3D tracking of zebrafish. The performance of the system is measured with respect to two detectors: a naive approach and a Faster R-CNN based fish head detector. The system reaches a MOTA of up to 77.6%. Links to the code and dataset is available at the project page https://vap.aau.dk/3d-zef

==> sections/contribution.tex <==
\begin{itemize}
    \item A new 3D tracking method for precise behavioral analysis of zebrafish.
    \item Publicly available source code for the proposed state-of-the-art 3D tracking system\footnote{\url{https://bitbucket.org/aauvap/zebrafish}}.
    \item A publicly available stereo dataset containing bounding box annotated sequences of zebrafish with IDs and tracks\footnote{\url{https://kaggle.com/aalborguniversity/zebrafish}}.
\end{itemize}


% Contributions from October 17 2019
\begin{itemize}
    \item Dataset 3D bounding-box niveau
    \item Dataset metrics
    \item System pipeline not requiring training data
    \item Re-ID for 3D tracklet association
\end{itemize}

%\begin{figure}[ht]
%    \centering
%    \begin{subfigure}[b]{0.45\textwidth}
%        \includegraphics[width=\textwidth]{figs/contr_ex.png}
%        \caption{Frame from a sequence with a school of \textit{small fish}.}
%        \label{fig:contr_ex}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.45\textwidth}
%        \includegraphics[width=\textwidth]{figs/contr_ex_annotated.png}
%        \caption{Same frame as above, but with annotations drawn on the image.}
%    \end{subfigure}
%    \caption{A frame example from the proposed dataset. The same frame is shown with and without annotations.}
%    \label{fig:contr_example}
%\end{figure}


==> sections/future.tex <==
The camera setup used to capture the proposed dataset has been developed in a way that allows for easy maintenance, adjustments, and replacement.
It is a permanent setup that will be used to monitor the various species that visit the area during the seasons. 
At the moment the three cameras are pointing diagonally downwards toward the riverbed, but there will be made ongoing modifications in order to capture different types of dataset, including stereo sequences.

The proposed dataset is part of an ongoing research project where data is logged 24 hours a day from all three cameras.
However, the recordings are stored in a compressed format in order to reduce the amount of data. 
In the future, the plan is to expand the current dataset with uncompressed recordings. 

The largest species that has been observed on the recordings is the harbor seal (\textit{Phoca vitulina}), which is a protected animal in national waters and of great interest for marine researchers.
The seal is not a part of the proposed dataset due to the few encounters so far, but hopefully will be in the future as more data is gathered and specific species are added to the dataset in close collaboration with local marine biologists.

==> sections/method.tex <==
\subsection{Object detection in 2D}

\subsubsection{Naive detection}

The naive detection approach is based on a set of basic computer vision operations.\\

Initially the background image, without any fish, is estimated by taking the median of $N$ images sampled uniformly across the video.

\textbf{Pre-processing:} The video is downsampled by a factor $k$ (\textit{currently by just picking every $n$ pixel}), and background subtraction is applied by calculating the absolute difference image, $|frame-bg|$, choosing max value across color channels,and  normalize the image $diff = 255 \times \frac{diff-min(diff)}{max(diff)-min(diff)}$ which results in range $[0;255]$. The resulting image is filtered with a $5\times 5$ median filter.

For the thresholding and detection steps, different approaches are used per view.\\

\textbf{Top view detection:} The frame is thresholded by using the middle point between the two modes in the image histogram. If the histogram is not bimodal, it is filtered with a $3\times 3$ mean filter, until it is bimodal.

The fish are detected by applying a skeletonization based approach. BLOBs are initially detected and filled, and the skeletonization approach of Zhang and Suen \fixme{Ref, skimage docu} is applied. The skeleton is analyzed in order to find the keypoints (head, tail, and junctions). This is done by convolving the frame with the kernel in Eq. \ref{eq:intPtMat}. All end points of the skeleton will have a value of 116, 117, 118, or 131, while junctions will have a value of 148, 149, 150, or 151. 
\begin{equation}\label{eq:intPtMat}
\begin{bmatrix}
1 & 1 & 1 & 1 & 1 \\
1 & 15 & 15 & 15 & 1 \\
1 & 15 & 100 & 15 & 1 \\
1 & 15 & 15 & 15 & 1 \\
1 & 1 & 1 & 1 & 1
\end{bmatrix}
\end{equation}


Each keypoint is assigned a weight, $w$,  which is the minimum eigenvalue of the covariance matrix of the BLOB coordinates extracted from a  $20\times 20$ window around the keypoint. The smallest eigenvalue is used, as it is assumed the variance will be smallest along the width of the head. The $w$ of the junction points are reduced by a factor of $2.5$, as they are usually larger than endpoint keypoints. 

Keypoints too close to each other are removed by applying non-maximal suppression (NMS). Each keypoint is assigned a bounding box of size $w\times w$, and kept if the bounding box does not overlap with any other keypoint by more than $nms_{thresh}$\% of the its area. In case there is an overlap, only the point with the largest $w$ is kept. 

Finally, all points with $w<1$ are discarded. The two keypoints with the largest distance between them are found, and the keypoint with largest $w$ is kept, together with the half of the keypoints, with the largest $w$ values. Each keypoint should ideally represent a fish head, and is kept as individual detections.\\



\textbf{Side view detection:} The image is first thresholded at the bin in the image histogram with the maximum total entropy. The entropy is modeled as \textit{black} and \textit{white} entropy for each non-zero bin. For bin $k$ the black and white entropy is calculated as shown in Eq. \ref{eq:blackEntropy}-\ref{eq:whiteEntropy}, resulting in the sets $B = \{b_0,b_1,..,b_{255}\}$ and $W = \{w_0,w_1,..,w_{255}\}$. These are combined as shown in Eq. \ref{eq:combinedEntropy} and the threshold, $t$, is set as in Eq. \ref{eq:entropyArgmin}. \fixme{Ref to Java code/paper}
\begin{equation}\label{eq:blackEntropy}
b_k = |\sum_{i = 0}^k \frac{h(i)}{c(i)} \log(\frac{h(i)}{c(i)})|
\end{equation}
\begin{equation}\label{eq:whiteEntropy}
w_k = |\sum_{i = k+1}^{255} \frac{h(i)}{1-c(i)} \log(\frac{h(i)}{1-c(i)})|
\end{equation}
\begin{equation}\label{eq:combinedEntropy}
E = B+W
\end{equation}
\begin{equation}\label{eq:entropyArgmin}
t = \argmin_x E(x)
\end{equation}
Where $h$ is the normalized histogram and $c$ is the cumulative histogram of $h$.\\


The BLOBs in the thresholded image are found through simple Connected Component Analysis (CCA). Only the $2N_{fish}$ largest BLOBs are kept, as long as the area of the BLOBs are larger than a predefined threshold. This allows for potential reflections being detected alongside the true detection of the fish. Otherwise the reflection might only be detected.

As it is not known where the head of the fish is, two points are saved as proxies for the head, together with the center-of-mass. If the width of the BLOB bounding box is larger than the height, the proxy points are $(min(x),\mu(y))$ and $(max(x),\mu(y))$, where $\mu$ is the arithmetic mean function. Otherwise, the proxy points are $(\mu(x),min(y))$ and $(\mu(x),max(y))$.\\

For both views the bounding boxes are determined per detection. The detected BLOBs are rotated so that they are parallel with the horizontal axis, and the bounding box of the rotated BLOB is calculated. This is done by determining the angle, $\theta$, between the eigenvectors of the covariance matrix of the zero-centered BLOB coordinates. \\


\textbf{Explain why the threshold methods are used. Better describe the weight used in the top view code, and the heuristic choices.}


\subsubsection{CNN detectors}
\textbf{Faster R-CNN}


\subsection{2D Tracklet Construction}

\subsubsection{Naive association}

As the zebrafish move erratically, it is not possible to set up a stable motion model. A naive tracking-by-detection approach is therefore applied. The tracking is done by constructing a distance matrix between each detection and the last detections of each current tracklet. The matrix is solved using the Hungarian algorithm \fixme{Ref}. 

Tracklets were deliberately constructed in a pessimistic way, where robust, but short, tracklets are encouraged. New detections are only assigned to a tracklet if it is within a predefined minimum distance. If a tracklet has not been assigned a detections within the last 10 concescutive frames, the tracklet is killed.

The $L_2$ distance between the head detections is used for the top view, and the Mahalanobis distance between the center-of-mass is used for the side view. The Mahalanobis distance is used as the zebrafish body is approximated to be elliptical in the side view, and it is more likely for the fish to move along the major axis (back/forth) than along the minor axis (up/down).\\



\subsection{3D Tracklet Association}
The 2D tracklets from each view are associated into 3D tracklets through a graph based approach. All 2D tracklets with more than $threshold$ detections are used. The 3D calibration and triangulation method from Pedersen et al. \fixme{Ref} is used, and the videos are temporally aligned.\\

\subsubsection{Graph construction}
A directed acyclic graph (DAG) is constructed. Each node consists of two 2D tracklets, one in each camera view and represents a 3D tracklet, and where each edge associates nodes where the 3D tracklet is based on the 2D tracklet in both nodes.\\

\textbf{Create nodes}: The graph nodes are constructed by processing each top view tracklet, and finding all side view tracklets which are intersecting in time, see Eq. \ref{eq:intersctingTracklets}.
\begin{equation}\label{eq:intersctingTracklets}
I = F_{T}\cap F_{S}
\end{equation}
Where $F_T$ and $F_S$ are the set of frames with detections in the top and side view tracklets, respectively. $I$ is the set of frames with detections in both views.\\

If $I=\emptyset$ the node is not created.

For each intersecting frame in $I$, denoted $f$, the 2D tracklets are triangulated, resulting in a 3D point of the zebrafish head, $p_f$, with a reproejction error $x_f$. Since the head is not directly assigned in the side view, the top view 2D point is triangulated with the two proxy points and the center-of-mass. $p_f$ therefore represents the point with the smallest reprojection error. In order to penalize large reprojection errors, a Gaussian CDF is utilized, based on the assumption that reprojection errors are normally distributed. This can be described as follows using set-builder notation Eq. \ref{eq:frameWeight}. 
\begin{equation}\label{eq:frameWeight}
V_w = \{ 1-\Phi(x_f \ | \ \mu_{err}, \sigma_{err}) \ | \ f \in I \wedge A(p_f)\}
\end{equation}
Where $\Phi$ is the Gaussian CDF of the normal distribution of reprojection errors, and $A$ is a boolean function which states whether $p_f$ is within the aquarium. \textit{Currently if A is not passed, a 0 is set instead of excluding the data point}\\

The per-frame weights in $V_w$ can be combined into a single weight for the entire node, using the weighting scheme in Eq. \ref{eq:nodeWeight}. This weighting scheme both considers the reprojection error, as well as the amount of intersecting frames. The median function is used instead of the mean function, in order to not let a few good triangulated points skew the weight.
\begin{equation}\label{eq:nodeWeight}
V = median(V_w) \times \frac{|V_w|}{|F_{T}\cup F_{S}|}
\end{equation}

The node is added to the DAG with the weight $V$, given that $V\neq 0$.\\


\textbf{Connect nodes:} The nodes in the DAG should be connected to all other nodes which build on one of the same 2D tracklets, as long as the other tracklets do not overlap temporally. An example is shown in Fig. \ref{}\fixme{TODO Make figure}. This is done by constructing the set of node pairs, $P$, from the set of nodes in the DAG, $N$. Node $n_i$ and $n_j$ is a node pair as long as they share a 2D tracklet, and the other 2D tracklet, denoted $t$, does not have a temporal overlap over $temp_{thresh}$, assuming $t_i$ start temporally earlier than $t_j$. Ideally the 2D tracklets should not overlap temporally. This can be represented in set-builder notation as in Eq. \ref{eq:nodePairSet}.
\begin{equation}\label{eq:nodePairSet}
P = \{(n_i, n_j) \ | \ n_i,n_j \in N \wedge O(n_i, n_j) \wedge T(n_i, n_j)\}
\end{equation}
Where $O$ checks that $t_i$ starts before $t_j$, and $T$ checks whether the temporal overlap threshold is fulfilled.\\

For each node pair in P the weight of the directed edge from $n_i$ to $n_j$ is based on the $L_2$ distance, $d$, between the last detection in $t_i$ and first detection in $t_j$, and the weights of the nodes, $V_i$ and $V_j$. For the top view the head is used, while for the side view the center-of-mass is used. The weight is calculated as shown in Eq. \ref{eq:edgeWeight}.
\begin{equation}\label{eq:edgeWeight}
E = (1-\Phi(d \ | \ \mu_{dist}, \sigma_{dist})) \times (V_i + V_j)
\end{equation}
Where $\Phi$ is the Gaussian CDF over the normal distribution of per frame zebrafish movement.\\

In case a node is not present in any node pairs, the node will be in the DAG, but have no edges.

% Go through the aforementioned map, and investigate tracklets with two or more nodes. The goal is to calculate aa directed edge between two nodes for tracklets in one view, denoted $n_1$ and $n_2$, that are assigned to the same tracklet in the other view. These tracklets are designated $t_1$ and $t_2$. It is assumed $t_1$ is temporally before $t_2$. $t_1$ and $t_2$ should ideally not overlap in time, but are allowed to overlap up to $threshold$ frames. The $L_2$ distance between the last detection in $t_1$ and first detection in $t_2$ is calculated and designated $d$. For the top view the head is used, while for the side view the center-of-mass is used.


\subsubsection{Graph evaluation} 
The 3D tracklets are extracted from the constructed DAG, by recursively finding the longest path in the graph. The longest path is the path throughout the DAG, which gives the highest value when summing all node and edge weights in the path.
After a path has been extracted and saved as a single 3D tracklet, the nodes used are removed from the DAG. This process is repeated until the DAG is empty. In case a 2D tracklet in the 3D tracklet is missing a detection in a frame, the 3D position cannot be assigned. Instead, only the known information of the 2D tracklet in question is assigned. The head position of side-view 2D tracklets is in this scenario assigned by assigning the proxy-point which minimize the $L_2$ distance to head positions in the consecutive frames. \fixme{unusure how to properly write this}

%Recursively extract longest paths in DAG. For each path extracted the nodes are removed, so they are not assigned multiple times.

%in case tracklets have been associated but in some frames one detection is missing in one view, the 3D position cannot be assigned. Instead the known information is added. 



\subsection{3D Track Construction}
3D track construction is performed in a greedy manner. A set of $N_{fish}$ tracklets are used as initial \textit{main tracklets}. The remaining tracklets, denoted \textit{gallery tracklets}, are assigned one by one to a single main tracklet, until no more tracklets can be assigned. This is repeated for $M$ different seed sets, and the resulting 3D tracks are consolidated.


\subsubsection{Initial tracklet selection}
The set of $N_{fish}$ main tracks are selected by finding the stable tracklets, that are temporally concurrent in time and span long time intervals. 
%Find all combinations of $N$ 3D tracklets which are all concurrent in time, and span the longest duration. 

For a 3D tracklet to be considered as a main track, it should be within the top $20\%$ tracklets, in regards to duration and number of detections. For each potential main track, the set of other 3D tracklets it is temporally concurrent with is considered. In the set, all possible $N_{fish}$ combinations are investigated. If the temporal overlap between all tracklets in the set are above a threshold, the combination is saved as a valid main tracklet set. The aforementioned threshold is the duration of the smallest potential main tracklet multiplied with a scale parameter (0.2). 

%For a 3D tracklet to be considered it should be within the top $20\%$ tracklets in regards to duration and number of detections. For each 3D tracklet find the set of other 3D tracklets it is concurrent with, in the sense of time spanned (and not frames with detections). For each set, investigate all possible combinations of size $N$. If the temporal overlap between all tracklets are above a set threshold, the combination is saved as a valid seed point. The aforementioned threshold is the duration of the $N\times mult$th tracklet timed with a parameter (0.2)

The valid tracklet set with the highest median temporal overlap is used to construct $N_{fish}$ full 3D tracks, using the greedy association scheme described in the following sections. If there are no valid combination of length $N_{fish}$, then no 3D tracklets are combined into 3D tracks.  


\subsubsection{Greedy association}
A greedy association algorithm is used, where each gallery tracklet is associated with a single main tracklet. The greedy part of the algorithm is the way the gallery tracklets are chosen: All gallery tracks are ranked in ascending order, by their shortest temporal distance to any main tracklet. If the gallery tracklet overlaps temporally with all main tracklets, it is relegated to the end of the list. After the gallery tracklet has been associated with a main track, the remaining gallery tracks are re-ranked based on the updated main tracklets. This way the main tracklets are ``grown'' into full tracks.\\

If at least one main tracklet does not overlap with the gallery tracklet, the association process is based on the spatio-temporal distances and using re-identification methods, between the gallery and non-overlapping main tracklets. Any temporally overlapping main tracklet is not considered.

In case the gallery tracklet temporally overlaps with all main tracklets, the internal spatio-temporal distances, re-identification methods, the amount of intersecting frames, and the ratio of intersecting frames compared to the total amount of detection in the gallery tracklet, are used.

All of these measured properties are denoted \textit{tracklet metrics}.\\

\textbf{Re-identification:} The re-identification step is built upon utilizing the recent advances within feature descriptors and metric/subspace learning based association methods, in the person re-identification field. In order to eliminate the need for prior training and annotated training data, the Local Maximal Occurrence (LOMO) feature descriptor and the Kernalized Discriminative Null Space (kDNS) subspace learning method are used \footnote{A discussion and comparison of different feature descriptors and association methods is presented in the supplemental materials.}. An RBF-kernel is used for the kDNS algorithm. The subspace transformation matrix of the kDNS algorithm is learned based on the detections in the main tracklets. For each main tracklet, the temporally closest detection to the gallery tracklet, is used as a \textit{probe}, in order to calculate the dissimilarity with each detection in the gallery tracklet. All dissimilarity values are combined into a dissimilarity matrix. The re-id step is only applied on the side-view in order to utilize the zerbafish stripe patterns. 

%\textbf{Re-identification:} The re-identification step is built upon using the Ensemble of Learned Features (ELF)\fixme{ref, check feature name} and Local Maximal Occurrence (LOMO) \fixme{ref} feature descriptors from size-normalized rotated bounding box of the fish detections, and applying metric learning person re-identification methods (Kernalized Discriminative Null Space (kDNS (with linear and RBF kernels)\fixme{Ref}, KISSME \fixme{ref}, improved KISSME (iKISSME) \fixme{ref}, LSSL \fixme{ref}, XQDA \fixme{ref}). These methods try to find a metric, or subspace, where the $L_2$ distance between two instances of the same class is minimized, while instances of different classes are maximized. This is typically done through estimating the Mahalanobis matrix, corresponding to a set of linear transformations applied to the (potentially PCA reduced) feature space, or by learning a subspace wherein the $L_2$ distance is measured. Simple distance measures ($L_1$, $L_2$, and Cosine Similarity) are also usable.  \textit{Describe a bit more which methods are used, what we do (e.g. what we calculate in ELF and LOMO, adn what we do not) etc.}

%The method-specific parameters are learned by using a balanced set of detections in the main tracklets. Detections of the gallery tracklets are compared to a \textit{probe} representation of the main tracklets, such as the mean or max of all features. For $L$ gallery tracklet detections, this results in a $L\times N_{fish}$ dissimilarity matrix. The $L$ gallery tracks detections are chosen based on how the gallery and main tracklets are temporally related. If the gallery tracklet occurs temporally after the main tracklet, the first $L$ detections in the gallery tracklet is used, if the gallery tracklet occurs after the main tracklet, the last $L$ detections are used, and if the tracklets are overlapping the $L$ detections are sampled throught the entire main tracklet (\textbf{should we set the sample interval to match the overlapping area with the gallery tracklet}). \textit{Write about re-training of Re-ID parameters, how the detections can be sampled at larger intervals and how the detections could also be sampled based on their orientations (if we use this)}\\

\textbf{Internal spatio-temporal distances:}  The internal spatio-temporal distances are determined through constructing a graph where each node is a detection in a frame, and the edge weight are the reciprocal spatial distance between the adjacent nodes (i.e. nodes at time $t$ are connected to all nodes at time $t+1$ and $t-1$)\fixme{Make figure}. The distances are calculated as the mean of the values when the graph switches from a detection in the gallery tracklet to the main tracklet, and vice versa. \\


%Rank unassigned tracklets based on their minimum temporal distance to any main track. If the tracklet overlaps temporally with all main tracks, it is relegated to the end of the list. Sorted in ascending order.

%For the selected unassigned tracklet, calculate the temporal distance, spatial distance, amount of intersecting frames, ratio of intersecting frame in comparison to the gallery track, Matrix of dissimilarity values from the Re-ID algorithm. 

%In case of the gallery tracklet temporally overlapping with all main tracks, the  internal temporal and spatial distances are calculated. This is done by constructing a graph where each node is a detection in a frame, and the edge weight are the reciprocal spatial distance between the adjacent nodes. The distances are then calculated as the mean of the values when the graph switches between tracks. 


%Potentially check Re-ID assignment first. If the probability of the most certain is more probable than the second most probable by a margin of $threshold$, then directly assign.

 

%\textbf{Re-identification}

%Either pre-defined bounding box size or use median width and height of the dataset

%\textbf{Feature descriptors}: LOMO, ELF\\

%\textbf{Classifiers}: KISSME, iKISSME, LSSL, XQDA, DNS, L1, L2, Cosine Dist.
 
 
%\textbf{training}: balanced dataset for training.  several methods

%\textbf{testing}: How to select which frames to use. Either just $K$ first or last frames, or use the orientation histogram Malte and I made? how to represent training data as a probe (mean, max, last)
 
 
 
\textbf{Association:} The different tracklet metrics are consolidated into a single assignment decision, through a global cost scheme. Each tracklet metric is normalized across main tracklets, into range $[0;1]$ and sum to 1. For the re-id dissimilarity matrix, each column (i.e. frame in the gallery track) are normalized, and each row averaged, in order to get a single re-id cost per main tracklet. These normalized values are interpreted as a cost of assigning the gallery tracklet to the respective main tracklets, that are not temporally overlapping, and summed into a final cost for each main tracklet. 

The gallery tracklet is associated with the main tracklet with the smallest cost, unless all main tracklet costs are within a small margin of each other (0.02), in which case the gallery tracklet is discarded. \\

% Calculate all the used metrics. At least one main track not overlapping: temporal, spatial, reid (only use data where the gallery track is not intersecting temporally with the main tracks).  All tracks overlapping: Intersection, internal spatial, internal temporal., intersection ratio (if any intersection).

%Convert all metrics to probabilities/costs, by dividing all values by the sum of the values.
%Convert the probabilities/costs into votes for which main track it should be assigned to by:

%1. Assign a metrics vote to the main track with the minimum probability/cost. 
%2. Add up all the probabilities/costs, normalize by the amount of metrics used

%option 2 is used. First it is checked if all votes are within a margin of each other. If so it isn't assigned to any main track. If not, the main track with the loves cost is assigned. 



\subsubsection{Interpolation}
After the different constructed main tracks have been consolidated into a single set, the missing 3D detections in the main tracks have to be filled in. This is done by linearly interpolating the 2D detections for the 3D track, and triangulating the 3D positions from these points.


==> sections/setup.tex <==
The setup used to record the proposed dataset was built entirely of off-the-shelf hardware.
An illustration of the setup is shown in \figref{setup}.
The two light panels are IKEA FLOALT of size $30\times 30$ cm with a luminous flux of 670 lumen and a color temperature of 4000K.
The top and front cameras are GoPro Hero 5 and GoPro Hero 7, respectively.
All the videos are recorded with a resolution of 2704x1520, 60 FPS, 1/60 $s$ shutter speed, 400 ISO, and a linear field of view.
Diffusion fabric was placed in front of the top light in order to reduce the amount of glare in the top view.
The test tank is a standard glass aquarium of size $30\times 30\times 30$ cm with a water depth of 15 cm.
Semi-transparent plastic was attached to three out of four of the window panes in order to reduce reflections. 
Furthermore, the front camera was placed orthogonally to the water level, which eliminated reflections from the water surface.
%The camera settings were chosen empirically and can be seen in \tableref{setup}. 
However, as the fish tank does not take up the entire image, the effective region of interest is lower than the specified camera resolution.
%\begin{table}[!ht]
%    \centering
%\begin{tabular}{cccccc}
%Resolution & FPS & Shutter  & ISO   & WB     & FoV    \\ \hline
%2704x1520  & 60 & 1/60  $s$    & 400   & Auto   & Linear
%\end{tabular}
%\caption{Camera settings.}
%\label{tab:setup}
%\end{table}
%The shutter speed was set as slow as possible, which allowed us to set the ISO low as well in order to reduce image noise.
%However, the low shutter speed introduces motion blur when the fish accelerates or swim with a certain velocity.
%This is a trade-off that depends strongly on the amount of light, velocity of the subjects and camera hardware.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/setup.png}
    \caption{Illustration of the test setup.}
    \label{fig:setup}
\end{figure}


==> sections/suppl_complexity.tex <==
\subsection{Occlusions}
The two views are not equal when it comes to occlusions.
Due to the social behavior of zebrafish they tend to swim in the same horizontal layer of the water column.
This is indicated by the graph in \figref{occ_ol}, where the occlusion lengths are displayed with respect to the proposed complexity measure. 
Data points are presented for all the recordings from both views, except Tst1 as it only contains a single fish. 
The dashed lines illustrate the mean occlusion lengths and they show that there is a significant difference between the two views.
In general, the occlusion events are longer in the front-view recordings and this makes robust tracking more difficult from this perspective.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/suppl/occ_ol.pdf}
    \caption{$\Psi$ is the proposed complexity measure based on the front- and top-view recordings. OL is the average length of occlusion events and the dashed lines show the mean OL for the two views. Tst1 is not included as it only contains a single fish.}
    \label{fig:occ_ol}
\end{figure}

The MOTA of the hypothetical oracle tracker is plotted against the proposed complexity measure in \figref{occ_mota}.
MOTA is calculated for the top- and front-view 2D tracklets as presented in \tableref{trackMeasuresTop} and \tableref{trackMeasuresFront}, respectively.
The tracking performance of the oracle tracker correlates well with the complexity in both views.
Notice the significant difference in performance of the tracker in the two views; the mean scores are MOTA$_{\text{top}}=86.0$ and MOTA$_{\text{front}}=75.5$ as illustrated by the two dashed lines.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/suppl/occ_mota.pdf}
    \caption{$\Psi$ is the proposed complexity measure based on the front- and top-view recordings. MOTA is based on the oracle tracker and the dashed lines show the mean MOTA for the two views. Tst1 is not included as it only contains a single fish.}
    \label{fig:occ_mota}
\end{figure}

